$S$-arithmetic (co)homology and $p$-adic automorphic forms

We study the $S$-arithmetic (co)homology of reductive groups over number fields with coefficients in (duals of) certain locally algebraic and locally analytic representations for finite sets of primes $S$. We use our results to construct eigenvarieties associated to parabolic subgroups at places in $S$ and certain classes of supercuspidal and algebraic representations of their Levi factors. We show that these agree with eigenvarieties constructed using overconvergent homology and that for definite unitary groups they are closely related to the Bernstein eigenvarieties constructed by Breuil-Ding.

==> format_basic.tex <==
\makeatletter

\def\emptycleardoublepage{\clearpage\if@twoside \ifodd\c@page\else
\thispagestyle{empty}%
\hbox{}\newpage\if@twocolumn\hbox{}\newpage\fi\fi\fi}

\makeatother
\newenvironment{nscenter}
 {\parskip=0pt\par\nopagebreak\centering}
 {\par\noindent\ignorespacesafterend}
\makeatletter
\newtheorem*{rep@theorem}{\rep@title}
\newcommand{\newreptheorem}[2]{%
\newenvironment{rep#1}[1]{%
 \def\rep@title{#2 \ref{##1}}%
 \begin{rep@theorem}}%
 {\end{rep@theorem}}}
\makeatother
\newtheoremstyle{note}%
{12pt}%
{9pt}%
{}%
{}%
{\bfseries}%
{.}%
{.5em}%
{}%
\newtheoremstyle{customnote}%
{12pt}%
{9pt}%
{}%
{}%
{\bfseries}%
{.}%
{.5em}%
{\def\temp{#3}\ifx\temp\empty\thmname{#1}\thmnumber{ #2}\else\thmnote{#3}\thmnumber{ #2}\fi}%
\newtheoremstyle{customnote*}%
{12pt}%
{9pt}%
{}%
{}%
{\bfseries}%
{.}%
{.5em}%
{\def\temp{#3}\ifx\temp\empty\thmname{#1}\else\thmnote{#3}\fi}%
\newtheoremstyle{thethm}%
{12pt}%
{3pt}%
{\itshape}%
{}%
{\bfseries}%
{.}%
{.5em}%
{}%
\theoremstyle{note}
\newtheorem{theorem}[equation]{Theorem}
\newtheorem*{theorem*}{Theorem}
\newreptheorem{theorem}{Theorem}
\newtheorem{proposition}[equation]{Proposition}
\newtheorem{lemma}[equation]{Lemma}
\newtheorem{claim}[equation]{Claim}
\newreptheorem{lemma}{Theorem}
\newtheorem{corollary}[equation]{Corollary}
\theoremstyle{note}
\newtheorem{remark}[equation]{Remark}
\newtheorem{fact}[equation]{Fact}
\newtheorem{example}[equation]{Example}
\newtheorem{notation}[equation]{Notation}
\newtheorem{exercise}[equation]{Exercise}
\newtheorem{prob}[equation]{Problem}
\newtheorem{definition}[equation]{Definition}
\newtheorem{conjecture}[equation]{Conjecture}
\newtheorem{question}[equation]{Question}
\newtheorem{question*}{Question}
\newtheorem{assumption}[equation]{Assumption}
\newtheorem{assumption*}{Assumption}
\newtheorem{construction}[equation]{Construction}
\theoremstyle{customnote}
\newtheorem{custom}[equation]{Theorem}
\theoremstyle{customnote*}
\newtheorem{custom*}{Theorem}
\renewenvironment{proof}[1][Proof]{\pushQED{\qed}\vspace{-0.3cm}\noindent\textit{#1. }}{\popQED}
\numberwithin{equation}{section}
\setlength\parindent{6pt}
\setlength{\parskip}{0.5em}
\setlist[itemize]{topsep=0pt, leftmargin=6mm}
\setlist[enumerate]{topsep=0pt, label={\rm (\roman*)}}
\newcommand{\itemnumber}[1]{{\rm (\romannum{#1})}}
\newcommand\blankpage{%
    \null
    \thispagestyle{empty}%
    \addtocounter{page}{-1}%
    \newpage}
\setlength{\abovedisplayskip}{1pt}
\setlength{\belowdisplayskip}{1pt}
\def\showproofstwo{0}

